Scaling Motion Forecasting Models with Ensemble Distillation

Motion forecasting has become an increasingly critical component of autonomous robotic systems. Onboard compute budgets typically limit the accuracy of real-time systems. In this work we propose methods of improving motion forecasting systems subject to limited compute budgets by combining model ensemble and distillation techniques. The use of ensembles of deep neural networks has been shown to improve generalization accuracy in many application domains. We first demonstrate significant performance gains by creating a large ensemble of optimized single models. We then develop a generalized framework to distill motion forecasting model ensembles into small student models which retain high performance with a fraction of the computing cost. For this study we focus on the task of motion forecasting using real world data from autonomous driving systems. We develop ensemble models that are very competitive on the Waymo Open Motion Dataset (WOMD) and Argoverse leaderboards. From these ensembles, we train distilled student models which have high performance at a fraction of the compute costs. These experiments demonstrate distillation from ensembles as an effective method for improving accuracy of predictive models for robotic systems with limited compute budgets.

==> sections/compare_results.tex <==
\begin{tabular}{cccc|cc}
\toprule
$\mathcal{L}_{gt}$ & $\mathcal{L}_{Distill}$ & $\mathcal{L}^{\mathds{1}}_{Distill}$  & \#ensembles &  minADE  ($\downarrow$) & mAP ($\uparrow$) \\ 
\midrule
\checkmark & & & 1 & 0.56 & 0.39 \\
\midrule
\checkmark & \checkmark & & 1 & 0.87 & 0.26 \\
\checkmark & & \checkmark & 1 & 0.56 & 0.40 \\
\midrule
\checkmark & \checkmark & & 28 & 0.53 & 0.41 \\
\checkmark &  & \checkmark & 28 & 0.61 & 0.38 \\
\bottomrule
\end{tabular}

==> sections/limitations.tex <==
\section {Limitations}

As in many machine learning applications, the best results in our experiments were obtained through manual tuning of parameters. One of the findings of this work is that there was no single choice of distillation loss functions and parameters that was optimal for all experiments. Our best results were obtained using large ensembles of models and the distillation loss as described in equation \ref{eq:approx_distill}. For smaller sized ensembles, however, the special case loss formulation in \ref{section:special} provides better results. One possible cause is that the shift in the distribution of the different sized teacher ensemble models requires re-tuning of the distillation parameters for each size. Please see the supplementary material for more experiments varying ensemble size with distillation.  Future work will focus on investigating these issues.

==> sections/loss_analysis.tex <==
\subsection{Distillation Loss Analysis}
We perform analysis of different formulations of our distillation loss. Here we ablate the use of the bijective mapping decribed in section \ref{section:special} denoted by $\pi_{1:1}$. In these experiments we train teachers and students with either 64 or 6 outputs. Where the number of outputs matches between teacher and student we apply the simplified bijection loss. Results are shown in 

\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cc|c|cc}
        \toprule
        $M_T$ & $N_S$ & $\pi_{1:1}$ &  minADE  ($\downarrow$) & mAP ($\uparrow$) \\ 
        \midrule
        6 & 6 & \checkmark & 0.64 & 0.37 \\
        64 & 64 & \checkmark & 0.55 & \textbf{0.43} \\
        64 & 6 & & \textbf{0.53} & \textbf{0.43} \\
        \bottomrule
        \end{tabular}
    }
    \caption{Comparison of the different distillation formulations in terms of trajectories fed into the model, output from the model and the distillation loss used for distillation on WOMD validation set. The number of teacher models $K=28$ to form the ensemble, the number of output modes from each teacher model is $N_T=64$ and the number of output trajectories from each student post NMS $M_S=6$ for metric computation.}
    \label{tab:compare_loss}
\end{table}

\begin{figure}[h]
\centering
\label{fig:results}
    \includegraphics[trim={0 0 0 2cm}, width=0.49\linewidth]{figures/soft_map_for_xent_vs_gmm_v7.png}
    \includegraphics[trim={0 0 0 2cm},width=0.49\linewidth]{figures/minade_for_xent_vs_gmm_v6.png}
\caption{ soft-mAP and MinADE metric results for the using students distilled with the bijective mapping $\pi_{1:1}$ (orange) and without (green) as a function of the number of teacher models $K$ in the teacher ensemble. } \label{fig:compare_for_xent_vs_gmm}
\end{figure}



 The results are tabulated in table \ref{tab:compare_loss}. We see it is better for distillation models to have teachers that are more expressive and output more modes in their distribution. Thus, $M_T = 64$ models output models with $M_T=6$. It is also interesting to note that while the overall best results are obtained by the model (row 3) that is allowed to learn the mapping between the modes of the student $N_S$ and the modes of the teachers $M_T$, the bijective mapping proposed in section \ref{section:special} does relatively reasonably and it not too far off in terms of the overall best performance (row 2).
 
 Figures \ref{fig:compare_for_xent_vs_gmm} show the results of experiments for two student models with the same architecture $N_S=64$, $M_S=64$ with teachers trained with $N_T=64$ in an ensemble. The number of teachers or ensemble size $K$ is varied from 1 ( self-distillation) to 28. The output number of modes from the ensemble is also NMS-ed down to $M_T=64$. We then either use the loss with $\pi_{1:1}$ (orange) or without (green) and see the effect of scaling up the ensemble size. We observe that for both of the loss formulations adding more models to the ensemble from which models are distilled, cause the performance to improve. In addition we see that using the bijective mapping  between teacher modes and student modes is better than having the model learn the mapping for small ensembles, but with a large enough ensemble size allowing the model to learn the mapping is better. This ultimately results in our state of the art model, although the deterministic bijective mapping is very competitive. 

